Explaining Image Classifiers Using Contrastive Counterfactuals in Generative Latent Spaces

Despite their high accuracies, modern complex image classifiers cannot be trusted for sensitive tasks due to their unknown decision-making process and potential biases. Counterfactual explanations are very effective in providing transparency for these black-box algorithms. Nevertheless, generating counterfactuals that can have a consistent impact on classifier outputs and yet expose interpretable feature changes is a very challenging task. We introduce a novel method to generate causal and yet interpretable counterfactual explanations for image classifiers using pretrained generative models without any re-training or conditioning. The generative models in this technique are not bound to be trained on the same data as the target classifier. We use this framework to obtain contrastive and causal sufficiency and necessity scores as global explanations for black-box classifiers. On the task of face attribute classification, we show how different attributes influence the classifier output by providing both causal and contrastive feature attributions, and the corresponding counterfactual images.

==> fig/Fig7.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.7\columnwidth]{fig/images/blonde_setmale.pdf}
\caption{Counterfactual image generation for computing contextual sufficiency and necessity scores. The context here is setting the attribute blond hair and we are computing scores for the attribute maleness. The attractiveness scores are at the lower left corner of each image. The original images are in the first row, followed by the counterfactual image had the context been set to high blondness. Finally, we generate the counterfactual image that has the attribute maleness set in this context.}
\label{fig:contextual_samples}
\end{figure}
